Differentially Private Assouad, Fano, and Le Cam

Le Cam's method, Fano's inequality, and Assouad's lemma are three widely used techniques to prove lower bounds for statistical estimation tasks. We propose their analogues under central differential privacy. Our results are simple, easy to apply and we use them to establish sample complexity bounds in several estimation tasks. We establish the optimal sample complexity of discrete distribution estimation under total variation distance and $\ell_2$ distance. We also provide lower bounds for several other distribution classes, including product distributions and Gaussian mixtures that are tight up to logarithmic factors. The technical component of our paper relates coupling between distributions to the sample complexity of estimation under differential privacy.

==> uniformity-lower_new.tex <==
\subsection{Sample Complexity Lower bounds for Uniformity Testing}\label{sec:lower-identity}

The first term is the lower bound without privacy constraints, proved in~\cite{Paninski08}. In this section, we prove the terms associated with privacy. 

The simplest argument is for $\ns \ge \frac{\ab}{\alpha^2}$, which hopefully will give the readers a sense of how coupling argument works. We consider the case of binary uniformity testing where the goal is to test whether the bias of a coin is $1/2$ or $\alpha$-far from $1/2$. This is a special case of uniformity testing for distributions over $[\ab]$ (when $\ab-2$ symbols have probability zero). This is strictly harder than the problem of distinguishing between $\Bern{1/2}$ and $\Bern{1/2+\alpha}$. The coupling given in Example~\ref{exm:coin} has expected hamming distance of $\alpha \ns$. Hence combing with Theorem~\ref{thm:le_cam}, by letting the RHS no larger than $\frac13$, we get a lower bound of $ \ns = \Omega\Paren{\min\Paren{\frac1{\dist\eps}, \frac1{\dist\delta} }} = \Omega({\frac{1}{\dist (\eps+\delta)}})$.

We now consider the cases $\ns \le \ab$ and $\ab< \ns \le \frac{\ab}{\alpha^2}$.

%The final term is a lower bound for testing identity to $\Bern{0.5}$, which is easier than uniformity testing by Theorem~\ref{thm:unif-identity}. 

To this end, we invoke our private LeCam's method, and design a hypothesis testing problem that will imply a lower bound on uniformity testing. The testing problem will be to distinguish between the following two cases. 

{\bf Case 1:} We are given $\ns$ independent samples from the uniform distribution $\unifab$.

{\bf Case 2:} Generate a distribution $\p$ with $\dtv{\p}{\unifab}\ge\dist$ according to some prior over all such distributions. We are then given $\ns$ independent samples from this distribution $\p$. 

From Theorem~\ref{thm:le_cam}, any lower bound for distinguishing between these two cases is a lower bound on uniformity testing problem. 

We now describe the prior construction for {\bf Case 2}, which is the same as considered by~\cite{Paninski08} for lower bounds on identity testing without privacy considerations. For each $\textbf{z} \in\{\pm1\}^{\ab/2}$, define a distribution $\p_{\textbf{z}}$ over $[\ab]$ such that 
\begin{align}
\p_{\textbf{z}}(2i-1) = \frac{1+\textbf{z}_i\cdot 2\dist}{\ab}, \text{ and } \p_{\textbf{z}}(2i) = \frac{1-\textbf{z}_i\cdot 2\dist}{\ab}.\nonumber
\end{align}
Then for any $\textbf{z}$, $\dtv{P_{\textbf{z}}}{\unifab}= \alpha$. For {\bf Case 2}, choose  $\p$ uniformly from these $2^{\ab/2}$ distributions. Let $Q_2$ denote the distribution on $[\ab]^\ns$ by this process. In other words, $Q_2$ is a mixture of product distributions over $[\ab]$. 

In {\bf Case 1}, let $Q_1$ be the distribution of $\ns$ $i.i.d.$ samples from $\unifab$. 

To obtain a sample complexity lower bound for distinguishing the two cases, we will design a coupling between $Q_1$, and $Q_2$, and bound its expected Hamming distance. While it can be shown that the Hamming distance of the coupling between the uniform distribution with any \emph{one} of the $2^{\ab/2}$ distributions grows as $\alpha\ns$, it can be significantly smaller, when we consider the mixtures. In particular, the following lemma shows that there exist couplings with bounded Hamming distance. 

\begin{lemma}\label{lem:coupling-hamming}
	There is a coupling between $\Xon$ generated by $Q_1$, and $\Yon$ by $Q_2$ such that 
\begin{center}
   $\expectation{\ham{\Xon}{\Yon}} \le C \cdot \dist^2 \min \{ \frac{\ns^2}{\ab}, \frac{\ns^{3/2}}{{\ab}^{1/2}} \}$.
%    \begin{cases}
%                                   8\frac{\ns^2\dist^2}{\ab}, & \text{when $m \le k$} \\
%                                    C\cdot \dist^2\frac{\ns^{3/2}}{{\ab}^{1/2}}, & \text{when $k< m \le \frac{k}{\alpha^2}$}.
%    \end{cases}
\end{center}
\end{lemma}
We refer the proof of the lemma to~\cite{AcharyaSZ18}. Now applying Theorem~\ref{thm:le_cam}, we get the bound in Theorem~\ref{thm:main-identity}.
%\begin{enumerate}
%	\item \newhz{For $m \le k$, $8\frac{\ns^2\dist^2}{\ab} = \Omega\Paren{\frac1{\eps}}$, implying $m = \Omega \Paren{\frac{\ab^{1/2}}{\alpha \eps^{1/2}}}$.}
%	\item \newhz{For $k< m \le \frac{k}{\alpha^2}$, $C\cdot \dist^2\frac{\ns^{3/2}}{{\ab}^{1/2}} = \Omega \Paren{\frac1{\eps}}$, implying $m = \Omega \Paren{\frac{\ab^{1/3}}{\alpha^{4/3}\eps^{2/3}}}$.}
%\end{enumerate}

%\begin{lemma}
%There is a coupling between $\Xon$  generated by $Q_2$, and $\Yon$ by $Q_1$ such that for 
%\[
%\expectation{\ham{\Xon}{\Yon}} \le
%\begin{cases}
%O\Paren{\dist^2\cdot\frac{\ns^2}{\ab}} & \ns\le \ab,\\
%O\Paren{\dist^2\cdot\frac{\ns^{3/2}}{\ab^{1/2}}}& k\le \ns\le \ab/\alpha^2,\\
%%O\Paren{\alpha\ns}&  \ab/\alpha^2\le\ns.
%\end{cases}
%\]
%\label{lem:coupling-uniform}
%\end{lemma}

%We can rewrite this result as
%\begin{align}
%\expectation{\ham{\Xon}{\Yon}} \le
%O\Paren{\min\left\{\dist^2\cdot\frac{\ns^2}{\ab}, \dist^2\cdot\frac{\ns^{3/2}}{\ab^{1/2}}, \alpha\ns\right\}}\label{eq:coup-ub}
%\end{align}
%	For the proof of this lemma, we can refer to lemma
%
%
%
%Using lemma~\ref{lem:coupling-uniform}, we can apply the coupling lower bound to prove the lower bound. 
%\begin{theorem}
%\[
%\Sitd\ge \Omega\Paren{\max\left\{\frac{\ab^{1/2}}{\alpha(\eps+\delta)^{1/2}}, \frac{\ab^{1/3}}{\alpha^{4/3}(\eps+\delta)^{2/3}}, \frac1{\dist(\eps+\delta)}\right\}}.
%\]
%\end{theorem}


%This is proved in the following lemma. 


%The construction of $Q_2$, and the proof of Lemma~\ref{lem:coup_unif} is slightly technical and is given in Section~\ref{app:lb-unif}.
%Assuming this lemma, by Theorem~\ref{thm:coupling}, we need $\expectation{\ham{\Xon}{\Yon}}=\Omega\Paren{\frac1{\eps+\delta}}$ to distinguish between $Q_1$, and $Q_2$. For this to hold, we need $\frac{\ns^2\dist^2}{\ab} = \Omega\Paren{\frac1{\eps+\delta}}$, which gives us 
%$\ns\ge \Omega\Paren{\frac{\sqrt \ab}{\dist\sqrt{\eps+\delta}}}$.




==> uniformity.tex <==
\section{$(\eps,\delta)$-DP uniformity testing}
\label{sec:identity}

\newhzn{
In this section, we give a proof sketch of sample complexity lower bound of uniformity testing. The full detail can be referred to~\cite{AcharyaSZ18}. The main result is the following. }

\begin{theorem}
\label{thm:main-identity}
The sample complexity of $(\eps,\delta)$-DP identity testing is
$$\Sutd = \Theta\Paren{\frac{k^{1/2}}{\dist^2}+\max\left\{\frac{\ab^{1/2}}{\alpha (\eps+\delta)^{1/2}}, \frac{\ab^{1/3}}{\alpha^{4/3} (\eps+\delta)^{2/3}}, \frac1{\dist(\eps+\delta)}\right\}}.$$
%
%Or we can write it according to the parameter range,
%\[
%    \Sit =
%    \begin{cases}
%                                   \Theta\Paren{\frac{\sqrt k}{\alpha^2} + \frac{\ab^{1/2}}{\alpha (\eps+\delta)^{1/2}}}, & \text{when $k = \Omega \Paren{\frac1{\alpha^4}}$ and $k = \Omega \Paren{\frac1{\alpha^2 (\eps+\delta)}}$,} \\
%              		  \Theta\Paren{\frac{\sqrt k}{\alpha^2} +\frac{\ab^{1/3}}{\alpha^{4/3} (\eps+\delta)^{2/3}}}, & \text{when $k = \Omega \Paren{\frac{\alpha}{(\eps+\delta)}}$ and $k = O \Paren{\frac1{\alpha^4}+\frac1{\alpha^2 (\eps+\delta)} }$,}\\
%              		               \Theta\Paren{\frac{\sqrt k}{\alpha^2} + \frac1{\alpha (\eps+\delta)}}, & \text{when  $k = O \Paren{\frac{\alpha}{(\eps+\delta)}}$.}\\ 
%    \end{cases}
%\]
\end{theorem}
We note that the lower bound is tight up to constant factors in all parameters. 

%In~\cite{AcharyaSZ18}, they show a reduction from identity to uniformity testing under differential privacy and design algorithms which achieve the matching upper bounds.
% 
%In this work, we focus on the lower bounds for identity testing. Since uniformity testing is a special case of identity testing, any lower bound for uniformity will port over to identity, and we give such bounds in Section~\ref{sec:lower-identity}.






